Possible studies at the first stage of the NICA collider operation with polarized and unpolarized proton and deuteron beams

This paper contains suggestions for experiments with usage of the Spin Physics Detector (SPD) at the first stage of the SPD NICA Programme developing at JINR. Double polarized pp-, dd- and pd- collisions at c.m.s. NN energies of 3.4-10 GeV, which will be accessible at the initial stage of experiments, allow one to study spin dependence of the NN interaction, search for multiquark states at double strangeness, charm and beauty thresholds, study the short-range structure of the deuteron. Double polarized pd scattering offer a possibility to test the Standard Model through the search for T-invariance violation.

==> Elkholy.tex <==
%\documentclass[a4paper]{panl}


\section{\bf On Measuring Antiproton-Production Cross Sections
%at NICA SPD
for Dark Matter Search
\protect
\footnote{This section is written by R.\,El-Kholy; {E-mail: relkholy@sci.cu.edu.eg}.}}
%\from{Astronomy Department, Faculty of Science, Cairo University, Giza, %Egypt, 12613}


\begin{abstract}
 Firm interpretation of the recent results from the AMS-02 and PAMELA spectrometers, regarding the antiproton yield in $p$-$p$ and $p$-$d$ collisions, has been hindered by uncertainties in production cross section, angular, and momentum spectra of the produced antiprotons. The proposed measurements of antiproton yield at the planned SPD experiment at the NICA collider could significantly contribute to enhancing the situation in favor of the search for dark matter WIMPs.
 
\end{abstract}
\vspace*{6pt}
\noindent

PACS: 95.35.+d, 95.55.Vj, 96.50.sb

%\label{sec:intro}
%\subsection{\textsc{Introduction}}
%\addcontentsline{toc}{section}{Introduction}
\vspace{0.5cm}

The dark matter (DM) problem is a long-standing puzzle in modern cosmology. Even though DM is known to make more than 26\% of the total energy-matter content of the Universe\cite{Ade2014}, we still have no confirmed conclusions about its identity. Evidence of DM is abundant and diverse, but mainly gravitational. The effects of DM have been observed in the rotation curves of galaxies, the mass discrepancy of galaxy clusters, and the lens-less gravitational lensing, among others\cite{Majumdar2014}. Perhaps most of our knowledge about DM properties was a product of the \emph{Bullet Cluster} event, where two galaxy clusters collided with one another. Astronomical observations and lensing analyses of the event assured astronomers that DM particles are only weakly interacting\cite{Clowe2006}. Once merely a tentative hypothesis, this has become widely accepted. Consequently, among many DM candidates, Weakly Interacting Massive Particles (WIMPs) became the most favored\cite{Buchmueller2017}.

There are several search approaches applied in the case of DM. Each of them has an underlying paradigm. The main three approaches are collider searches, direct detection, and indirect detection. Collider searches are based on the hypothesis that DM particles can be pair-produced in collisions of Standard-Model (SM) particles, either directly or via a mediator. Direct detection experiments try to measure the recoil energy of DM particles colliding with SM nuclei. Indirect detection seeks to prove the hypothesis that DM particles decay and pair-annihilate producing SM particles as final products\cite{Buchmueller2017}. Thus, astrophysical searches try to accurately measure rare fluxes in Cosmic Rays (CRs), in order to detect a secondary anomalous signature of DM. To identify an anomalous signal, it is crucial to first subtract other ordinary astrophysical sources. Secondary CR fluxes are produced in collisions of primary CRs on Inter-Stellar Medium (ISM). In particular, secondary antiprotons are produced in proton-nucleus, nucleus-proton, and nucleus-nucleus collisions. 

During the last two decades, two satellite-borne experiments, namely, PAMELA\cite{Adriani2014} and AMS-02\cite{Aguilar2013}, have measured the secondary antiproton flux and antiproton-to-proton ratio with unprecedented accuracy, covering a wide energy range. The AMS-02 experiment has measured antiproton-to-proton ratio with an accuracy higher than 95\% for kinetic energies from 1 to 450 GeV\cite{Aguilar2016}. However, we still cannot come to firm conclusions about any exotic signal because the AMS-02 measurements are still surrounded with several sources of uncertainties as shown in Fig.\ref{fig:uncertainties}. These sources stem from uncertainties on: (i) the primary spectra slopes at high energies, (ii) the solar modulation at lower energies, (iii) the propagation parameters in the galactic environment, and (iv) the antiproton-production cross sections. The first two can be relatively reduced through new AMS-02 measurements. The third can be minimized via parameter variation. However, the last of these sources is the most significant and ranges between 20\% and 50\%, depending on the energy\cite{Giesen2015}.

\begin{figure}[ht]
%	\includegraphics[width=\linewidth]{Elkholy/uncertainties.pdf}
	\includegraphics[width=\linewidth]{Elkholy/uncertainties.eps}
	\caption{The combined total uncertainty on the predicted secondary $\bar{p}/p$ ratio superimposed to the PAMELA and the AMS-02 data. Each envelope accounts for uncertainties enclosed in it; such that the green band is the total band of all four sources of uncertainty\cite{Giesen2015}.}
	\label{fig:uncertainties}
\end{figure}

In addition to the scarcity of cross-section measurements of antiproton-production, most available datasets date back to before 1980, and did not account for hyperon decay to antiprotons\cite{Mauro2014}. Thus raising the need for new measurements of antiproton-production cross sections. The kinematic phase-space coverage required to catch up to the AMS-02 measurements has been outlined\cite{Donato2017}. Here, we affirm the capability of the Spin Physics Detector (SPD), planned at the NICA collider currently under construction at JINR, to make a sizable contribution to the desired measurements\cite{Guskov2019,Alexakhin2020}.

\label{sec:pbar-production}
%\subsection{\textsc{Antiproton Production Cross Sections.}}
\subsection{{Antiproton Production Cross Sections}}
The contribution of each interaction channel of primary CRs with ISM to the production of secondary antiprotons depends on the abundances of different nuclei in both CRs and ISM. Based on the abundances outlined in\cite{Guskov2019}, the most dominant channel of antiproton production would be proton-proton collisions, followed by proton-helium, and proton-deuteron collisions, respectively. Other nucleus-nucleus collisions have a negligible contribution. In addition to different production channels, there are also different production mechanisms. The dominant mechanism is the direct production. However, antiprotons are also produced via decay of anti-baryons; namely, antineutrons, and the $\bar{\Lambda}$ and $\bar{\Sigma}^{-}$ hyperons. The overall antiproton-production cross section can be expressed as\cite{Winkler2017}
\begin{equation}
	\sigma_{\bar{p}} = \sigma_{\bar{p}}^{0} (2+\Delta_{\text{IS}}+2\Delta_{\Lambda}),
\end{equation}
where $\Delta_{\text{IS}} = \sigma_{\bar{n}}^{0}/\sigma_{\bar{p}}^{0} - 1$ is the isospin enhancement factor of antineutron direct production, and $\Delta_{\Lambda} = \sigma^{\Lambda}_{\bar{p}}/\sigma_{\bar{p}}^{0}$ is the hyperon factor, assuming $\sigma_{\bar{n}}^{\Lambda} = \sigma_{\bar{p}}^{\Lambda}$.

The currently-available data on proton-proton collisions is extremely scarce. It is graphically summarized in Fig.\ref{fig:datasets}, in terms of transverse momentum, $p_{T}$, and the radial-scaling variable, $x_{R}$, which is given by\cite{Mauro2014}
\begin{equation}
	x_{R}=\dfrac{E_{\bar{p}}^{*}}{E_{\bar{p}.\text{max}}^{*}},
\end{equation}
where $E_{\bar{p}}^{*}$ is the antiproton energy, and $E_{\bar{p}.\text{max}}^{*}$ is the maximal energy it can acquire, both in the CM frame. The maximal antiproton energy can be obtained by\cite{Mauro2014}
\begin{equation}
	E_{\bar{p}.\text{max}}^{*}=\dfrac{s-8m_{p}^{2}}{2\sqrt{s}}.
\end{equation}
Moreover, most of these datasets date back to before 1980, and thus do not include a hyperon-decay feed-down. As for datasets on other production channels, they are essentially non-existent. The first ever proton-helium dataset has been released by the LHCb collaboration in 2018\cite{Aaij2018}.

\begin{figure}[ht]
%	\includegraphics[width=\linewidth]{Elkholy/datasets_CM.pdf}
	\includegraphics[width=\linewidth]{Elkholy/datasets_CM.eps}
	\caption{The available data on $d^{3}\sigma_{pp\rightarrow\bar{p}}/dp^{3}$ in the $p_{T}-x_{R}$ space\cite{Mauro2014}.}
	\label{fig:datasets}
\end{figure}

In addition to measuring the cross sections of direct antiproton production, it is necessary to accurately estimate the hyperon factor, $\Delta_{\Lambda}$, as well. The hyperon factor can be expressed as\cite{Winkler2017}
\begin{equation}
\label{eq:hyperon-factor}
\Delta_{\Lambda} = \frac{\bar{\Lambda}}{\bar{p}} \times \text{BF}_{\bar{\Lambda}\to \bar{p} \pi^+}
+  \frac{\bar{\Sigma}^-}{\bar{p}} \times \text{BF}_{\bar{\Sigma}^-\to \bar{p} \pi^0},
\end{equation}
where $\bar{\Lambda}/\bar{p}$ and ${\bar{\Sigma}}^-/\bar{p}$ are the hyperon to promptly-produced antiproton ratios, and $\text{BF}_{\bar{\Lambda}\to \bar{p} \pi^+}$ $= 0.639\pm0.005$ and $\text{BF}_{\bar{\Sigma}^-\to \bar{p} \pi^0}=0.5157\pm0.0003$ are the branching fractions of the corresponding decays. While there are some existing data on the ratio $\bar{\Lambda}/\bar{p}$, there is not any data on the ratio $\bar{\Sigma}^{-}/\bar{p}$; and it is only estimated based on the symmetry argument that $\bar{\Sigma}^{-}/\bar{\Lambda}=0.33$\cite{Kappl2014}. Thus, expression \eqref{eq:hyperon-factor} can be rewritten as
\begin{equation}
\Delta_{\Lambda}=(0.81\pm0.04)\times\bar{\Lambda}/\bar{p}.
\end{equation}
Even existing data on the ratio $\bar{\Lambda}/\bar{p}$ has a high energy-dependent uncertainty ranging from 12\% to 18\%\cite{Winkler2017}.

From all of the above, the need for new measurements, of the antiproton-production cross sections and hyperon-to-antiproton production ratios, becomes clear. The phase space that requires coverage in order to bridge the gap between antiproton data and the AMS-02 measurements has been outlined. Fig.\ref{fig:spd-coverage} shows it in terms of transverse momentum and the radial-scaling variable, where the areas within the contours need to be covered with uncertainty no more than 3\%, while the areas outside the contours require coverage with uncertainty no more than 30\%\cite{Donato2017}.

\begin{figure}[ht]
	\includegraphics[width=\linewidth]{Elkholy/SPD_coverage.pdf}
	\caption{The kinematic range accessible to the SPD\cite{Alexakhin2020} superimposed on the required measurement range to match the AMS-02 accuracy\cite{Donato2017}.}
	\label{fig:spd-coverage}
\end{figure}
\break
\label{sec:nica-spd}
%\subsection{\textsc{NICA SPD Contribution.}}
\subsection{{NICA SPD Contribution}}
The SPD detector is planned to operate at the NICA collider currently under construction at JINR\cite{Savin2015}. Polarized proton and deuteron beams will be used. The $pp$ collisions are expected to reach $\sqrt{s}=27$ GeV, and a luminosity of $5\times10^{30}$ cm$^{-2}$s$^{-1}$ should be achieved\cite{Meshkov2019}. Preliminary MC results using PYTHIA8\cite{Sjoestrand2015} show that the antiproton-production cross section in $pp$ collisions multiplied by the average antiproton-multiplicity in this energy range is on the level of a few millibarns\cite{Guskov2019}, corresponding to a production rate $>10^{5}$ s$^{-1}$. Thus, the measurements will not be hindered by statistical uncertainty. The $4\pi$ angular acceptance of the SPD will also allow access to a wider kinematic range, in comparison to fixed-target experiments. Fig.\ref{fig:spd-coverage} shows the kinematic range accessible to the SPD based on a preliminary MC study\cite{Alexakhin2020}, superimposed on the required measurement range to match the AMS-02 accuracy.

The time-of-flight system of the SPD detector will enable particle identification. In addition, reconstruction of secondary-vertices will allow the study of secondary hyperon decays\cite{Alexakhin2020}. Thus, the SPD can also contribute to measurement of the $\bar{\Lambda}/\bar{p}$ ratio, where Fig.\ref{fig:hyperons-range} shows the energy range accessible to the SPD.

\begin{figure}[ht]
	\includegraphics[width=\linewidth]{Elkholy/hyperon.pdf}
	\caption{$\bar{\Lambda}/\bar{p}$ ratio in proton-proton collisions as measured by several experiments\cite{Winkler2017}. The range of $\sqrt{s}$ accessible at the NICA SPD is indicated at the lower left part\cite{Alexakhin2020}.}
	\label{fig:hyperons-range}
\end{figure}

\label{sec:summary}
%\subsection{\textsc{Summary.}}
\subsection{{Summary}}
The Spin Physics Detector can make a sizable contribution to the search of physics beyond the Standard Model. The SPD can measure energy and angular distributions of antiprotons produced in proton-proton and proton-deuteron collisions both directly and from the decays of $\bar{\Lambda}$ and $\bar{\Sigma}^{-}$ hyperons in the kinematic range starting from the threshold, for the astrophysical searches for dark matter. The collider mode and the geometry of the SPD detector provide a unique possibility to study the production of antiprotons at high transverse momenta which is unavailable for fixed-target experiments. The possibility for NICA to operate with beams of light nuclei, such as $^{3}He$ and $^{4}He$, could extend this program.

%\label{sec:ref}
%\bibliographystyle{pepan}
%\bibliography{ref}

%\end{document} 


==> Kostenko-15fbr.tex <==

\section{\bf {Study of inelastic d-d and p-d interactions for observation of
neutron-proton system under strong compression}
\protect\footnote {B.F.\,Kostenko; {E-mail: bkostenko@jinr.ru}}}

\begin{abstract}

In this experimental proposal, we consider a possibility of registering light dibaryons at the NICA SPD facility, experimental and theoretical indications of the existence of which were previously obtained at JINR. The main attention is paid to the description of the observable effects, as well as the requirements for measuring instruments necessary for their successful detection.
\end{abstract}

\vspace*{6pt}
\noindent

PACS: 24.85.+p, 13.88.+e, 13.85.Fb 

\label{sec:introa}
\subsection{Introduction}
At present, there are different theoretical indications that cold nucleonic matter under strong compression should undergo phase transitions, see, e.g., \cite{PhaseTran}. Experiments at NICA MPD will be devoted to the search for signs of these transitions, in which the manifestations of the transformations of the nucleon phase into quark-gluon one, as well as other transitions, is expected to be seen in collisions of heavy nuclei. Unfortunately, traditional nuclear physics, as well as astrophysical restrictions on the equation of state for cold dense matter, do not yet give direct indications of the need to take into account such processes \cite{Astro}. A similar situation has arisen in the description of small nucleon systems, which can be used as the basis for the microscopic theory of phase transitions in nuclear matter. Thus, it has long been suggested that various multibaryon states can exist in nature in the form of a configurational admixture together with ordinary nuclei \cite{Matv-Sorba}. At the same time, models continued to develop, suggesting that nucleons in nuclei can also retain their individuality even in very exotic high-momentum states \cite{GG}.
An attempt to find experimental manifestations of the multiquark component in the wave function of atomic nuclei was undertaken in the frame of the flucton model\cite{Efremov,BLT}. In parallel, the model of short-range correlations according to which, to explain the same processes, the nucleon models, taking into account the high-momentum component of the wave function of nuclei, were also quite suitable \cite{FrStr}.

Experiments on the NICA MPD facility should in the future answer some of the questions associated with the problem of phase transitions of nucleonic matter into other forms of nuclear substance at high densities, which can be achieved in collisions of heavy nuclei accelerated to relativistic velocities. The theory of these phenomena is extremely difficult, so that the interpretation of the obtained experimental data may turn out 
to be highly uncertain. In this regard, it is of particular interest to study the transitions of nucleonic matter to other states, which can occur in few-nucleon systems. Drawing an analogy with the theory of the formation of an electron-ion plasma, it can be argued that, in this respect, 
knowledge of the characteristics of few-nucleon systems under conditions of strong compression can contain information as indispensable as knowledge of the ionization characteristics of atoms for building a theory of ordinary plasma.

\eject

\label{sec:idea2}
\subsection{Search for new dibaryons at the NICA SPD facility}
There are a number of theoretical and experimental indications of the existence of light dibaryon excitations in 2-nucleon systems \cite{Kostenko,Troyan,Baldin}.
An analysis of the experimental data suggests the possible observation of events, the cross sections of which in a certain kinematic region are comparable to the cross sections of hard elastic nucleon-deuteron collisions.
For example, in \cite{Baldin} a peak was observed, which is interpreted to date as a quasi-free knockout by the target deuteron of a nucleon from the incident deuteron  in the reaction d $ + $ d $ \to $ d $ + $ X.
However, its large width can hardly be explained only by the internal motion of nucleons in the deuteron being destroyed.
At the same time, kinematic analysis shows \cite{Kostenko} that  scattering processes with the participation of virtual dibaryons preexisting in the incident deuteron in a virtual form before the collision can also contribute to the observed peak.
In experiments \cite{Troyan}, where the effective masses of two-nucleon systems formed after the emission of several (up to 5) pions from highly excited neutron-proton systems were measured, there are indications of the observation of narrow dibaryons, the masses of which can be described by a simple formula \cite{Kostenko} $M_n = M_d +10.08 n$ MeV, where
$M_d = 1875.6$ MeV is the value of deuteron mass\footnote{Hereinafter, the system of units is used, in which $ c = 1 $.}.
It can hardly be interpreted as a mere coincidence that the broadening of the peak caused by the ``quasi-free'' nucleon knockout in the experiment \cite{Baldin} can also be explained \cite{Kostenko} by scattering d $ + $ d $ \to $ d $ + $ d $ ^ * $ with the participation of the same dibaryons as in the experiment \cite{Troyan}. Of course, these arguments can only be considered as indirect evidence in favor of the existence of light dibaryons. 
On the other hand, it must be emphasized that the criticism of Troyan's experiment presented in \cite{Abramov}  also does not look convincing enough.
Firstly, in  \cite{Troyan} a larger number of events were studied than in \cite{Abramov}; secondly, in \cite{Abramov} , events with a poorer ``cooling'' of a highly excited dibaryon were used, i.e. the work is based on events with fewer secondary pions emitted by a highly excited dibaryonic system.
And finally, even in spite of all that, significant variations in the measured cross sections were observed in \cite{Abramov}, which can hardly be explained by simple statistical fluctuations.
The above facts suggest that light dibaryons could have been present in a sufficiently large number already in some of the earlier experiments, but were not recognized due to insufficient spectral resolution of the corresponding experimental facilities.
Drawing an analogy with the history of discoveries associated with the invention of the microscope, we can say that a medium that can contain a large number of interesting microscopic objects is  presumably known, but a device that allows them to be clearly seen has not yet been created.
Below we shall consider  the demands  that would have to be advanced to an experimental setup so that it could be used to obtain unambiguous answers to all the above questions. 

In experiments on colliding beams of deuterons with momenta of the same modulus, the energy $ q_0 $ transferred in the reaction d + d $ \to $ d + d $ ^ * $ from one of the deuterons to the dibaryon being produced is
\begin{equation}\label{q0CollBeams}
{q_0} = \frac{{M_*^2 - M_d^2}}{{4{E}}}, 
\end{equation}
where $ {E} = \sqrt {P ^ 2 + M_d ^ 2} $ is the deuteron energy in the laboratory coordinate system (l.c.s.).
For the $ n- $th excited level of the dibaryon 
$ {M_ *} = {M_d} + n \varepsilon $.
Here $ \varepsilon $ is the distance between the levels, which we will take equal to 10 MeV \cite{Kostenko}. The relation (\ref {q0CollBeams}) allows one to estimate the influence of the instability of the beam energy $ E $ on the accuracy of determining the value of $ \varepsilon $.
For this purpose, let us bring into correspondence the spread in energy $ \Delta E $ of deuterons in beams and the inaccuracy of setting the level number $ 0 < \delta <1 $, which will describe the deviation of the measured level energy from its exact value, referred to $ \varepsilon $.
Substitution of $ E \to E + \Delta E $ and $ n \to n + \delta n $ into the relation (\ref {q0CollBeams}) gives a quadratic equation for $ n $, which determines the highest level for which the uncertainty in the distance between adjacent levels is does not yet exceed the value of $ \delta $:
\begin{equation}\label{delta} 
\frac{{\Delta E}}{E} =  \frac{{2{M_d} + (2n + \delta )\varepsilon }}{{2{M_d}n + {n^2}\varepsilon }} \delta.
\end{equation}
For $ n \varepsilon \ll {M_d} $, this relation is reduced to a directly proportional relationship between the relative fluctuation of the beam energy and the relative error in measuring the distance between adjacent levels, caused by these fluctuations:
\[\delta  \approx \frac{{\Delta E}}{E}n.\]
It turns out to be rather weak (so far, the influence of the beam momentum spread on the accuracy of measuring the $ M _ * $ dibaryon mass is not taken into account).
For example, for $ \Delta E = 100 $ MeV, the error in determining the energy of the tenth level of a dibaryon is only 1 MeV for the momentum of colliding beams at the level of 10 GeV in l.c.s.

It is also useful to have the correspondence between the 4-momentum $ q $ transferred to the nascent dibaryon, which can be measured experimentally, and the relativistic Mandelstam  variable $ t \equiv q_0 ^ 2 - \mathbf {q} ^ 2. $
One can make sure after elementary but cumbersome calculations that for the experiments with colliding beams the following simple formula holds:
\begin{equation}\label{tCollBeams}
 t=2(E{q_0} - P{q_\parallel }).
\end{equation}
Here $ q_ \parallel $ is longitudinal, i.e. directed along the beams$'$ axis, the component of the momentum transfer, which is directly responsible for the excitations.
%CHECK
%It can be seen from (\ref{tCollBeams}) that the processes of dibaryon production from a kinematic
It can be seen from (\ref{tCollBeams}) that the processes of dibarion production from a kinematic
%point of %view are possible at both negative and positive, as well as zero values ​​of 
point of view are possible at both negative and positive, as well as zero values of
%the variable $t$, which seems to be extremely unlikely.
the varibale $t$, which seems to be extremely unlikely.
%It is clear that the dynamic theory of the processes should be based on a relativistic-invariant
It is clear that the dynamic theory of the processe should  be based on the relativistic-invariant
%amplitude %using the variable $t$, since the fact of dibaryon production does not depend on the frame 
amplitude using the variable $t$, since the fact of dibarion production does not depend on the frame
in which it is registered. In the absence of such a theory, the answer 
to the question of whether the dibaryons under consideration are produced,
%CHECK
%for example, at zero values ​​of the variable $t$, can only be given by experiment. 
for example, ar zero values of the variable $t$, can only be given by experiment.
Since the relativistic-invariant amplitude also depends on the Mandelstm variable 
$s$, the search for the region of localization of dibaryons should also be accompanied
by a variation in the momentum of deuterons in colliding beams.


Traditionally, formula (\ref{q0CollBeams}) is used to identify resonances, in which $ M_* $ is the effective mass of  decay products of a resonance.
An individual resonance can be seen if an error of its mass determining, which includes its own width, and also takes into account the measurement errors of the momenta of its decay products, is significantly less than distances to adjacent levels. It is clear that, to recognize resonances, one can also use the  relationship (\ref{tCollBeams}), in which resonances are seen as separate lines. However, to formulate the requirements for the experimental setup,
the most appropriate is a method of  resonance recognition directly based on the quantities to be measured. Indeed, resonances, as well as the degree of reliability of their recognition, can also be seen on graphs of the dependence $ q_\bot (q_\parallel) $ with a direct indication of the measurement errors of  longitudinal $ q_ \parallel $ and perpendicular $ q_\bot $ components of the momentum transfer. The exact analytical dependence $ {q_ \bot} ({q_\parallel}) $ for colliding beams with equal momenta has the form
\begin{equation}\label{q_t(q_||)}
{q_\bot }({q_\parallel }) = \sqrt {{{\left( {\frac{{4{E^2} + M_*^2 - M_d^2}}{{4E}}} \right)}^2} - M_*^2 - {{(P - {q_\parallel })}^2}}. 
\end{equation}
\begin{figure}
\begin{center}
\includegraphics[width=127mm]{q_t_on_qL3.eps}
%\includegraphics[width=127mm]{Kostenko/q_t_on_qL3.eps}
\end{center}
\caption{\small 
Dependence of the transverse momenta of light dibaryons on their longitudinal momenta measured in MeV for an experiment with colliding beams with  $P=3$ GeV. The uppermost curve corresponds to the first excited level, and the lowest one corresponds to the tenth level. 
}\label{q_t_on_qL}
\end{figure}


%CHECK
This dependece is shown in Fig. \ref{q_t_on_qL}, for the supposed theoretical
values ​​of the masses of dibaryons and $P=3$ GeV. In a real experiment, values ​​of the momenta of decay products of a dibaryon should be measured. For light dibaryons, these are the momenta $ \mathbf {p}_n $ and $ \mathbf {p}_p $ of the secondary neutron and proton. The transverse component of the momentum transferred to the dibaryon is equal to the transverse component of the total momentum of the secondary nucleons 
$ q_\bot = p_{n \bot} + p_{p \bot} $, which is known with the measurement accuracy $ \Delta p_{n, p \bot} = \Delta p_{n \bot} + \Delta p_{p \bot} $. In addition, the nonzero fluctuation of the transverse momentum of the beam $ \Delta P_\bot $ makes a contribution to the measurement error of the transverse momentum transfer.
Thus, the total measurement error of the transverse component of the momentum transfer is calculated by the formula
$$\Delta q_\bot = \Delta p_{n\bot} + \Delta p_{p\bot} + \Delta P_\bot.$$ 
Similarly, taking into account that $ q_\parallel = P- (p_{n \parallel} + p_{p \parallel}) $, we have
$$ \Delta q_\parallel = \Delta p_{n \parallel} + \Delta p_ {p \parallel} + \Delta P_\parallel, $$
where $ \Delta P_\parallel $ is a value of the beam momentum fluctuations.

In paper \cite{Baldin}, in which the light dibaryons could be observed at $t = $ -0.5 GeV$^2$, interactions  of deuterons with momentum $ P = $ 8.9 GeV with a stationary deuteron target were used.
The colliding beam experiments at $ | P | = $ 3 GeV correspond to the deuteron momentum $ P = $ 11.3 GeV in experiments with the stationary target, which is close to the value in \cite{Baldin}.



Using the formulas (\ref{q0CollBeams}) and (\ref{tCollBeams}),
it can be verified that the kinematics of colliding beams corresponds to similar events at $ q_\parallel = $ 100 $ \pm $ 20 MeV.
In its turn, the formula (\ref{q_t(q_||)}) tells us that at $ q_\parallel  = $ 100 MeV the value of $ q_\bot $ will be  755.8 MeV for elastic d-d scattering, 743.2MeV for scattering with excitation of the first level, 730.3 MeV for scattering with excitation of the second level, ... 631.0 MeV -- for the tenth level. In this range, the distances between the levels grow as follows:  12.3, 12.6, 12.9, ... 14.9, 15.3 MeV. Thus, it can be seen that the measurement accuracy of the transverse momentum at a level of 3 MeV is quite enough to register all the dibaryons described above.

To estimate the required accuracy of measuring the longitudinal component of the momenta of the secondary particles, the dependence (\ref{q_t(q_||)}) should be reversed, expressing $ P-q_\parallel $ in terms of $ q_\bot $.
One can check that the distances in the horizontal direction
between the levels of dibaryons shown in Fig. \ref{q_t_on_qL}, in this case only slightly more than 3 MeV at full longitudinal
momentum $ P-q_\parallel $ of the decay products at a level of 3000 MeV. This dictates very high requirements  both for the measurement accuracy of the longitudinal components of  momentum of the secondary particles and the degree of monochromaticity of the beam  -- at the level of $10 ^{- 4}$. 
Nevertheless, even in this respect, the experiments with colliding beams have significant advantages in relation to experiments with the stationary target.
In the latter case, a similar experiment would require increasing relative accuracy by a factor of 7, because of the larger momentum $ P $ of the accelerated beam and also because of a different analytical dependence $ q_\bot (q_\parallel ) $.  

The requirements for the accuracy of measuring the longitudinal component of the momentum transfer very fast decrease with decreasing momentum of the colliding beams. So, if it is equal to 1 GeV, then the required relative accuracy becomes equal to 10$^{-2}$.
%CHECK
%Since the exact range of values ​​of the Mandelstam variable $s$, within which the production of
Since the exact range of values of the Mandelstam variable $s$, within which the production of 
%light dibaryons is possible, we do not know, then it makes sense to set up an experiment 
light dibaryons is possible, we do not know, then it makes sense to set up an experiment
%even at lower than in the experiment \cite{Baldin} values ​​of $s$.
even at lower than in the experiment \cite{Baldin} values of $s$.

Fig.\ref{q_t_on_qL} suggests the possibility of searching for any dibaryons, including heavier
ones, the existence of which quark models  predict. For this, it is enough to use the fact 
of a distinct concentration events near some line $ {q_ \bot }({q_\parallel }) $, described by formula (\ref{q_t(q_||)}), which should be very similar to those shown in Fig.\ref{q_t_on_qL}.









==> Kostenko-8fbr.tex <==

\section{\bf {Study of inelastic d-d and p-d interactions for observation of
neutron-proton system under strong compression}
\protect\footnote{ This section is written by B.F.\,Kostenko, {E-mail: bkostenko@jinr.ru}}}
\begin{abstract}
%В данном экспериментальном предложении рассматривается возможность регистрации на установке %NICA SPD легких дибарионов, экспериментальные и теоретические указания на существование %которых были ранее получены в ОИЯИ.  Основное внимание  уделяется описанию возможных %наблюдаемых эффектов, а также формулировке требований к измерительной аппаратуре, необходимых %для их успешной  регистрации. 
%\vspace{0.2cm}

In this experimental proposal, we consider a possibility of registering light dibaryons at the NICA SPD facility, experimental and theoretical indications of the existence of which were previously obtained at JINR. The main attention is paid to the description of the observable effects, as well as the requirements for measuring instruments necessary for their successful detection.
\end{abstract}

\vspace*{6pt}
\noindent

PACS: 24.85.+p, 13.88.+e, 13.85.Fb 

\label{sec:introa}
\subsection{Introduction}
At present, there are different theoretical indications that cold nucleonic matter under strong compression should undergo phase transitions, see, e.g., \cite{PhaseTran}. Experiments at NICA MPD will be devoted to the search for signs of these transitions, in which the manifestations of the transformations of the nucleon phase into quark-gluon one, as well as other transitions, is expected to be seen in collisions of heavy nuclei. Unfortunately, traditional nuclear physics, as well as astrophysical restrictions on the equation of state for cold dense matter, do not yet give direct indications of the need to take into account such processes \cite{Astro}. A similar situation has arisen in the description of small nucleon systems, which can be used as the basis for the microscopic theory of phase transitions in nuclear matter. Thus, it has long been suggested that various multibaryon states can exist in nature in the form of a configurational admixture together with ordinary nuclei \cite{Matv-Sorba}. At the same time, models continued to develop, suggesting that nucleons in nuclei can also retain their individuality even in very exotic high-momentum states \cite{GG}.
An attempt to find experimental manifestations of the multiquark component in the wave function of atomic nuclei was undertaken in the frame of the flucton model\cite{Efremov,BLT}. In parallel, the model of short-range correlations according to which, to explain the same processes, the nucleon models, taking into account the high-momentum component of the wave function of nuclei, were also quite suitable \cite{FrStr}.

Experiments on the NICA MPD facility should in the future answer some of the questions associated with the problem of phase transitions of nucleonic matter into other forms of nuclear substance at high densities, which can be achieved in collisions of heavy nuclei accelerated to relativistic velocities. The theory of these phenomena is extremely difficult, so that the interpretation of the obtained experimental data may turn out 
to be highly uncertain. In this regard, it is of particular interest to study the transitions of nucleonic matter to other states, which can occur in few-nucleon systems. Drawing an analogy with the theory of the formation of an electron-ion plasma, it can be argued that, in this respect, 
knowledge of the characteristics of few-nucleon systems under conditions of strong compression can contain information as indispensable as knowledge of the ionization characteristics of atoms for building a theory of ordinary plasma.



\label{sec:idea2}
\subsection{Search for new dibaryons at the NICA SPD facility}
There are a number of theoretical and experimental indications of the existence of light dibaryon excitations in 2-nucleon systems \cite{Kostenko,Troyan,Baldin}.
An analysis of the experimental data suggests the possible observation of events, the cross sections of which in a certain kinematic region are comparable to the cross sections of hard elastic nucleon-deuteron collisions.
For example, in \cite{Baldin} a peak was observed, which is interpreted to date as a quasi-free knockout by the target deuteron of a nucleon from the incident deuteron  in the reaction d $ + $ d $ \to $ d $ + $ X.
However, its large width can hardly be explained only by the internal motion of nucleons in the deuteron being destroyed.
At the same time, kinematic analysis shows \cite{Kostenko} that  scattering processes with the participation of virtual dibaryons preexisting in the incident deuteron in a virtual form before the collision can also contribute to the observed peak.
In experiments \cite{Troyan}, where the effective masses of two-nucleon systems formed after the emission of several (up to 5) pions from highly excited neutron-proton systems were measured, there are indications of the observation of narrow dibaryons, the masses of which can be described by a simple formula \cite{Kostenko} $M_n = M_d +10.08 n$ MeV, where
$M_d = 1875.6$ MeV is the value of deuteron mass\footnote{Hereinafter, the system of units is used, in which $ c = 1 $.}.
It can hardly be interpreted as a mere coincidence that the broadening of the peak caused by the ``quasi-free'' nucleon knockout in the experiment \cite{Baldin} can also be explained \cite{Kostenko} by scattering d $ + $ d $ \to $ d $ + $ d $ ^ * $ with the participation of the same dibaryons as in the experiment \cite{Troyan}. Of course, these arguments can only be considered as indirect evidence in favor of the existence of light dibaryons. 
On the other hand, it must be emphasized that the criticism of Troyan's experiment presented in \cite{Abramov}  also does not look convincing enough.
Firstly, in  \cite{Troyan} a larger number of events were studied than in \cite{Abramov}; secondly, in \cite{Abramov} , events with a poorer ``cooling'' of a highly excited dibaryon were used, i.e. the work is based on events with fewer secondary pions emitted by a highly excited dibaryonic system.
And finally, even in spite of all that, significant variations in the measured cross sections were observed in \cite{Abramov}, which can hardly be explained by simple statistical fluctuations.
The above facts suggest that light dibaryons could have been present in a sufficiently large number already in some of the earlier experiments, but were not recognized due to insufficient spectral resolution of the corresponding experimental facilities.
Drawing an analogy with the history of discoveries associated with the invention of the microscope, we can say that a medium that can contain a large number of interesting microscopic objects is  presumably known, but a device that allows them to be clearly seen has not yet been created.
Below we shall consider  the demands  that would have to be advanced to an experimental setup so that it could be used to obtain unambiguous answers to all the above questions. 

In experiments on colliding beams of deuterons with momenta of the same modulus, the energy $ q_0 $ transferred in the reaction d + d $ \to $ d + d $ ^ * $ from one of the deuterons to the dibaryon being produced is
\begin{equation}\label{q0CollBeams}
{q_0} = \frac{{M_*^2 - M_d^2}}{{4{E}}}, 
\end{equation}
where $ {E} = \sqrt {P ^ 2 + M_d ^ 2} $ is the deuteron energy in the laboratory coordinate system (l.c.s.).
For the $ n- $th excited level of the dibaryon 
$ {M_ *} = {M_d} + n \varepsilon $.
Here $ \varepsilon $ is the distance between the levels, which we will take equal to 10 MeV \cite{Kostenko}. The relation (\ref {q0CollBeams}) allows one to estimate the influence of the instability of the beam energy $ E $ on the accuracy of determining the value of $ \varepsilon $.
For this purpose, let us bring into correspondence the spread in energy $ \Delta E $ of deuterons in beams and the inaccuracy of setting the level number $ 0 < \delta <1 $, which will describe the deviation of the measured level energy from its exact value, referred to $ \varepsilon $.
Substitution of $ E \to E + \Delta E $ and $ n \to n + \delta n $ into the relation (\ref {q0CollBeams}) gives a quadratic equation for $ n $, which determines the highest level for which the uncertainty in the distance between adjacent levels is does not yet exceed the value of $ \delta $:
\begin{equation}\label{delta} 
\frac{{\Delta E}}{E} =  \frac{{2{M_d} + (2n + \delta )\varepsilon }}{{2{M_d}n + {n^2}\varepsilon }} \delta.
\end{equation}
For $ n \varepsilon \ll {M_d} $, this relation is reduced to a directly proportional relationship between the relative fluctuation of the beam energy and the relative error in measuring the distance between adjacent levels, caused by these fluctuations:
\[\delta  \approx \frac{{\Delta E}}{E}n.\]
It turns out to be rather weak (so far, the influence of the beam momentum spread on the accuracy of measuring the $ M _ * $ dibaryon mass is not taken into account).
For example, for $ \Delta E = 100 $ MeV, the error in determining the energy of the tenth level of a dibaryon is only 1 MeV for the momentum of colliding beams at the level of 10 GeV in l.c.s.

It is also useful to have the correspondence between the 4-momentum $ q $ transferred to the nascent dibaryon, which can be measured experimentally, and the relativistic Mandelstam  variable $ t \equiv q_0 ^ 2 - \mathbf {q} ^ 2. $
One can make sure after elementary but cumbersome calculations that for the experiments with colliding beams the following simple formula holds:
\begin{equation}\label{tCollBeams}
 t=2(E{q_0} - P{q_\parallel }).
\end{equation}
Here $ q_ \parallel $ is longitudinal, i.e. directed along the beams$'$ axis, the component of the momentum transfer, which is directly responsible for the excitations.
%CHECK
%It can be seen from (\ref{tCollBeams}) that the processes of dibaryon production from a kinematic
It can be seen from (\ref{tCollBeams}) that the processes of dibarion production from a kinematic
%point of %view are possible at both negative and positive, as well as zero values ​​of 
point of view are possible at both negative and positive, as well as zero values of
%the variable $t$, which seems to be extremely unlikely.
the varibale $t$, which seems to be extremely unlikely.
%It is clear that the dynamic theory of the processes should be based on a relativistic-invariant
It is clear that the dynamic theory of the processe should  be based on the relativistic-invariant
%amplitude %using the variable $t$, since the fact of dibaryon production does not depend on the frame 
amplitude using the variable $t$, since the fact of dibarion production does not depend on the frame
in which it is registered. In the absence of such a theory, the answer 
to the question of whether the dibaryons under consideration are produced,
%CHECK
%for example, at zero values ​​of the variable $t$, can only be given by experiment. 
for example, ar zero values of the variable $t$, can only be given by experiment.
Since the relativistic-invariant amplitude also depends on the Mandelstm variable 
$s$, the search for the region of localization of dibaryons should also be accompanied
by a variation in the momentum of deuterons in colliding beams.


Traditionally, formula (\ref{q0CollBeams}) is used to identify resonances, in which $ M_* $ is the effective mass of  decay products of a resonance.
An individual resonance can be seen if an error of its mass determining, which includes its own width, and also takes into account the measurement errors of the momenta of its decay products, is significantly less than distances to adjacent levels. It is clear that, to recognize resonances, one can also use the  relationship (\ref{tCollBeams}), in which resonances are seen as separate lines. However, to formulate the requirements for the experimental setup,
the most appropriate is a method of  resonance recognition directly based on the quantities to be measured. Indeed, resonances, as well as the degree of reliability of their recognition, can also be seen on graphs of the dependence $ q_\bot (q_\parallel) $ with a direct indication of the measurement errors of  longitudinal $ q_ \parallel $ and perpendicular $ q_\bot $ components of the momentum transfer. The exact analytical dependence $ {q_ \bot} ({q_\parallel}) $ for colliding beams with equal momenta has the form
\begin{equation}\label{q_t(q_||)}
{q_\bot }({q_\parallel }) = \sqrt {{{\left( {\frac{{4{E^2} + M_*^2 - M_d^2}}{{4E}}} \right)}^2} - M_*^2 - {{(P - {q_\parallel })}^2}}. 
\end{equation}
\begin{figure}
\begin{center}
%\includegraphics[width=127mm]{q_t_on_qL3.eps}
\includegraphics[width=127mm]{Kostenko/q_t_on_qL3.eps}
\end{center}
\caption{\small 
Dependence of the transverse momenta of light dibaryons on their longitudinal momenta measured in MeV for an experiment with colliding beams with  $P=3$ GeV. The uppermost curve corresponds to the first excited level, and the lowest one corresponds to the tenth level. 
}\label{q_t_on_qL}
\end{figure}


%CHECK
%This dependece is shown in Fig. \ref{q_t_on_qL}, for the supposed theoretical
%values ​​of the masses of dibaryons and $P=3$ GeV. In a real experiment, values ​​of the momenta of decay products of a dibaryon should be measured. For light dibaryons, these are the momenta $ \mathbf {p}_n $ and $ \mathbf {p}_p $ of the secondary neutron and proton. The transverse component of the momentum transferred to the dibaryon is equal to the transverse component of the total momentum of the secondary nucleons 
$ q_\bot = p_{n \bot} + p_{p \bot} $, which is known with the measurement accuracy $ \Delta p_{n, p \bot} = \Delta p_{n \bot} + \Delta p_{p \bot} $. In addition, the nonzero fluctuation of the transverse momentum of the beam $ \Delta P_\bot $ makes a contribution to the measurement error of the transverse momentum transfer.
Thus, the total measurement error of the transverse component of the momentum transfer is calculated by the formula
$$\Delta q_\bot = \Delta p_{n\bot} + \Delta p_{p\bot} + \Delta P_\bot.$$ 
Similarly, taking into account that $ q_\parallel = P- (p_{n \parallel} + p_{p \parallel}) $, we have
$$ \Delta q_\parallel = \Delta p_{n \parallel} + \Delta p_ {p \parallel} + \Delta P_\parallel, $$
where $ \Delta P_\parallel $ is a value of the beam momentum fluctuations.

In paper \cite{Baldin}, in which the light dibaryons could be observed at $t = $ -0.5 GeV$^2$, interactions  of deuterons with momentum $ P = $ 8.9 GeV with a stationary deuteron target were used.
The colliding beam experiments at $ | P | = $ 3 GeV correspond to the deuteron momentum $ P = $ 11.3 GeV in experiments with the stationary target, which is close to the value in \cite{Baldin}.



Using the formulas (\ref{q0CollBeams}) and (\ref{tCollBeams}),
it can be verified that the kinematics of colliding beams corresponds to similar events at $ q_\parallel = $ 100 $ \pm $ 20 MeV.
In its turn, the formula (\ref{q_t(q_||)}) tells us that at $ q_\parallel  = $ 100 MeV the value of $ q_\bot $ will be  755.8 MeV for elastic d-d scattering, 743.2MeV for scattering with excitation of the first level, 730.3 MeV for scattering with excitation of the second level, ... 631.0 MeV -- for the tenth level. In this range, the distances between the levels grow as follows:  12.3, 12.6, 12.9, ... 14.9, 15.3 MeV. Thus, it can be seen that the measurement accuracy of the transverse momentum at a level of 3 MeV is quite enough to register all the dibaryons described above.

To estimate the required accuracy of measuring the longitudinal component of the momenta of the secondary particles, the dependence (\ref{q_t(q_||)}) should be reversed, expressing $ P-q_\parallel $ in terms of $ q_\bot $.
One can check that the distances in the horizontal direction
between the levels of dibaryons shown in Fig. \ref{q_t_on_qL}, in this case only slightly more than 3 MeV at full longitudinal
momentum $ P-q_\parallel $ of the decay products at a level of 3000 MeV. This dictates very high requirements  both for the measurement accuracy of the longitudinal components of  momentum of the secondary particles and the degree of monochromaticity of the beam  -- at the level of $10 ^{- 4}$. 
Nevertheless, even in this respect, the experiments with colliding beams have significant advantages in relation to experiments with the stationary target.
In the latter case, a similar experiment would require increasing relative accuracy by a factor of 7, because of the larger momentum $ P $ of the accelerated beam and also because of a different analytical dependence $ q_\bot (q_\parallel ) $.  

The requirements for the accuracy of measuring the longitudinal component of the momentum transfer very fast decrease with decreasing momentum of the colliding beams. So, if it is equal to 1 GeV, then the required relative accuracy becomes equal to 10$^{-2}$.
%CHECK
%Since the exact range of values ​​of the Mandelstam variable $s$, within which the production of
Since the exact range of values of the Mandelstam variable $s$, within which the production of 
%light dibaryons is possible, we do not know, then it makes sense to set up an experiment 
light dibaryons is possible, we do not know, then it makes sense to set up an experiment
%even at lower than in the experiment \cite{Baldin} values ​​of $s$.
even at lower than in the experiment \cite{Baldin} values of $s$.

Fig.\ref{q_t_on_qL} suggests the possibility of searching for any dibaryons, including heavier
ones, the existence of which quark models  predict. For this, it is enough to use the fact 
of a distinct concentration events near some line $ {q_ \bot }({q_\parallel }) $, described by formula (\ref{q_t(q_||)}), which should be very similar to those shown in Fig.\ref{q_t_on_qL}.





%\bibliography{Kostenkoeng}


%\end{document}



==> Uzhinsk.tex <==

\section{\bf Problems of soft $pp$ interactions
\protect\footnote{This section is written by A.\,Galoyan  and V.\,Uzhinsky.
%;{E-mail: uzhinsky@jinr.ru}.
}}
%\from{$^{a}$\,Veksler and Baldin Laboratory of High Energy Physics, Joint Institute for Nuclear Research,%
%	Dubna, Moscow region, 141980 Russia}
%\vspace{-3mm}
%\from{$^{b}$\,Laboratory of Information Technologies, Joint Institute for Nuclear Research,
%	Dubna, Moscow region, 141980 Russia}

\begin{abstract}
% Russian translation of the abstract

%Предлагаются эксперименты, направленые на решение трех основных проблем физики мягких
%$pp$ взаимодействий: понимание/описание спектров барионов в $pp$ соударениях, эволюция
%$<P^2_T>$ -- $x_F$ корреляций с ростом энергии и двух-частичные $P_T$ корреляции рожденных
%частиц.

\vspace{0.2cm}

Experiments are proposed directed on solution of three main problems of physics of soft
$pp$ interactions: understanding/description of baryon spectra in $pp$ collisions, evolution
of $<P^2_T>$ -- $x_F$ correlations with energy growth and two-particle $P_T$ correlations.

\end{abstract}
\vspace*{6pt}

\noindent
PACS: 24.10.Lx, 13.85.Ni, 14.20.-c  

Description of proton spectra in hadron-nucleon interactions is a long standing problem of high
energy physics. By tradition, three reggeon phenomenology is used for its solution at $x_F \rightarrow$ 
1 (see Ref.~\cite{KaidalovPhysRep}). Especially, it is assumed that the three pomeron graph (PPP) is 
responsible for the high mass diffraction dissociation. The non-vacuum reggeon -- two pomeron's graph
(RPP) is connected with so-called low mass diffraction dissociation. The three non-vacuum reggeon's
graph (RRR) gives a contribution at $x_F \geq$ 0.8. A.B.~Kaidalov and O.I. Piskunova 
\cite{KaidalovPiskunova} proposed a method of the spectra description in the central region in 
the framework of the Quark-Gluon-String  model. Up to now various Monte Carlo models cannot describe 
the spectra sufficiently well \cite{Uzhi2014}. All of them are used the LUND fragmentation scheme
\cite{LUND} for a treatment of decays of quark-diquark strings. An example of the description is presented in
Fig.~1 where Pythia 6.4 \cite{Pythia6_4} and Geant4 FTF model's predictions are shown.

The Geant4 FTF model \cite{Geant4FTF} considers RRR graphs. As seen, the Pythia model gives abnormal 
humps at $y\sim$ 1.7 and 2.3 at $P_{lab}=$ 158 and 400 GeV/c, correspondently. Thus, detailed 
experimental data at low energies, where the diffractions are dominant processes, are highly 
desired for a development of the theoretical models.

The most impressive experimental data on $pp$ interactions were presented in the last decade by 
the NA61/SHINE collaboration for $\sqrt{s_{NN}}=$ 6.2, 7.6, 8.8, 12.3 and 17.3 GeV \cite{NA61pp}. 
It is pitty, but the data are not sufficiently detailed. Before there were data at $P_{lab}=$ 12
and 24 GeV/c \cite{PP12_24}. They were based on low statistics according to a modern point of view.

On the whole, we can say that the FTF model of Geant4 toolkit describes quite well the multiplicities and
kinematical spectra of produced particles in proton-proton interactions in a wide laboratory energy range 
from 1 GeV up to 1000 GeV.

\begin{figure}[bth]
	\begin{center}
		\resizebox{5in}{2in}{\includegraphics{Uzhinsk/GalUzhFig1.png}}
		\resizebox{5in}{2in}{\includegraphics{Uzhinsk/GalUzhFig1.png}}
		\vspace{-3mm}
		\caption{Distributions of $\pi^\pm$ and protons on rapidity in the
			center-of-mass system of $pp$ interactions at $P_{lab}$= 158 and 400 GeV/c. Points are experimental
			data \protect{\cite{NA61pp,LEBC-EHS400}} without systematical errors. Solid and dashed curves are FTF and Pythia 6.4 
			model calculations.
		}
	\end{center}
	\label{Fig1}
	\vspace{-5mm}
\end{figure}

Another problem, recognized by us, was observed in $<$$P^2_T$$>$ -- $x_F$ correlations in $pp$ interactions.  
The NA61/SHINE collaboration did not provide corresponding experimental data for the correlations,
though, they can be extracted in principle. The NA49 collaboration presented the needed data \cite{NA49pi,NA49pn,NA49K} 
only at the page -- \newline  http://spshadrons.web.cern.ch/ppdata.html. 
The data are very different from analogous data by
the LEBC-EHS collaboration \cite{LEBC-EHS400} at $\sqrt{s_{NN}}=$ 27.5 GeV. The models cannot describe 
the last data quite well.
\begin{figure}[bth]
	\begin{center}
		\resizebox{5in}{2in}{\includegraphics{Uzhinsk/GalUzhFig2.png}} % 6 3
		\vspace{-3mm}
		\caption{$<P^2_T>$ -- $x_F$ correlations in $pp$ interactions at $\sqrt{s_{NN}}$=17.3 GeV. Points are
			the NA49 data \protect{\cite{NA49pi,NA49pn,NA49K}}. Solid and dashed lines are FTF and Pythia 6.4 model calculations.
		}
	\end{center}
	\label{Fig2}
	\vspace{-5mm}
\end{figure}

As seen in Fig.~2, the models describe the general behaviour of the data except the correlations for protons. Predictions
of the models are close to each other and to the data for $\pi^+$, $\pi^-$, $K^+$ and $K^-$ mesons at
$\sqrt{s_{NN}}=$ 17.3 GeV. The FTF model overestimates the correlations for protons at $x_F \geq$ 0.2, and
does not reproduce the hump at $x_F \sim$ 0. The Pythia model gives the hump, but it is essential lower than
the experimental data. In other regions of $x_F$, the Pythia model does not describe the shape of the data.
At higher energy, the situation becomes worse for the proton correlation. This shows that both models
have a problem with baryon production in $pp$ interactions.

It is interesting to look at evolution of the correlations with energy. In Fig.~3 we present $<P^2_T>$ -- $x_F$ correlations
at various energies. As seen, there is a smooth evolution, though there is a change of process contributions with energy in
the FTF model. Quark exchange processes and one-vertex diffractions dominate at low energies. At higher energies, the diffraction
is stay on the same lavel, but an yield of non-diffractive processes is increased.
\begin{figure}[bth]
	\begin{center}
		\resizebox{4in}{4in}{\includegraphics{Uzhinsk/GalUzhFig3.png}} % 6 3
		\vspace{-3mm}
		\caption{$<P^2_T>$ -- $x_F$ correlations in $pp$ interactions at $\sqrt{s_{NN}}$=3.2, 6.3, 8.8 and 17.3 GeV
			(lines from bottom to top). Points are the NA49 data \protect{\cite{NA49pi,NA49pn,NA49K}}. Lines are FTF 
			model calculations.
		}
	\end{center}
     \label{Fig2a}
	\vspace{-5mm}
\end{figure}

In order to clarify a nature of the correlations, we propose to study two-particle $P_T$ correlations
in soft interactions. The correlation can be also studied by current experiments at RHIC and the LHC.

As known, two-particle correlations were intensively used in the past at study of particles and
jets in high energy physics (see, for example, \cite{Phenix200,ATLAS_2T,ATLAS_pPb,ATLAS_5T,ALICE}). 
At the present time, there 
are well developed methods of jet recognition \cite{anti-kt1,anti-kt2} and analysis of thier properties.
More complicated situation takes place at sufficiently lower energies, especially for 
nucleus-nucleus interactions, when hard jets cannot be produced. Though, some methods of high 
energies can be adjusted for lower energies. Instead of jets with high $P_T$, one can choose
as a trigger a particle of any type in an event. An associated particle can be choosen in the 
same manner in the event, where the trigger paticle is produced.

In general, two-particle $P_T$ correlation function can be determined as:
\begin{equation}
C(\vec P^{tr}_T,\vec P^{as}_T)=\frac{1}{N_{tr}} \ \frac{d\ N(tr,as)}{d^2P^{tr}_T\ d^2 P^{as}_T},
\label{Eq6}
\end{equation}
where $\vec P^{tr}_T$ is a transverse momentum of a trigger particle. $\vec P^{as}_T$ is a
transverse momentum of an associated particle. $N_{tr}$ is a number of the trigger 
particles. $N(tr,as)$ is a number of pairs -- trigger particles and associated particle
having pre-determined values of $\vec P^{tr}_T$ and $\vec P^{as}_T$.

The function $C$ is a function of 4 independent variables. Though, accounting azimuthal symmetry
of interactions of unpolarized particles there must be only 3 independent variables. We propose to
use as the variables the module of transverse momentum of the trigger particle ($|\vec P^{tr}_T|$), 
and 2 projections of the vector $\vec P^{as}_T$ on the direction of the vector $\vec P^{tr}_T$,
and on the direction perpendicular to $\vec P^{tr}_T$ (see Fig.~4). In Fig.~4
we choose $\Lambda$ as a trigger particle, and $K$-meson or $\pi$-meson as associated particles.  

\begin{minipage}{5.5cm}
	\resizebox{2in}{2in}{\includegraphics{Uzhinsk/GalUzhFig4.png}}
	\centerline{Fig. 4} 
\addtocounter{figure}{1}
	\label{Fig16}
%	\addtocounter{figure}{1}
\end{minipage}
\begin{minipage}{7.4cm} % 10
	\begin{equation}
	P^{as}_{T,L}\ =\ \vec P^{as}_T \cdot \vec P^{tr}_T/|\vec P^{tr}_T|,
	\label{Eq7}
	\end{equation}
	\begin{equation}
	P^{as}_{T,T}\ =\ |\vec P^{as}_T \otimes \vec P^{tr}_T|/|\vec P^{tr}_T|
	\label{Eq8}
	\end{equation}
	
	Instead of calculations of scalar and vector products, one can use the following method:
	Determine the azimuthal angle of flying of the trigger particle -- $\phi = \arctan{P^{tr}_{T,y}/P^{tr}_{T,x}}$.
	Make the Euler transform of the coordinate system, and find new components of $\vec P^{as}_T$. 
	\begin{eqnarray}
	P^{as}_{T,x'}=\ P^{as}_{T,x}\cdot \cos{\phi}\ +\ P^{as}_{T,y}\cdot \sin{\phi}, \label{Eq9}\\
	P^{as}_{T,y'}= -P^{as}_{T,x}\cdot \sin{\phi}\ +\ P^{as}_{T,y}\cdot \cos{\phi}. \label{Eq10label} 
	\end{eqnarray}
\end{minipage}

%\vspace{-5mm}

It is obvious, that the new components of $\vec P^{tr}_T$ will be $P^{tr}_{T,x'}=|\vec P^{tr}_{T}|$
and $P^{tr}_{T,y'}=0$. In the following, we will omit subscripts "$T$", and apostrophes of $x$ and $y$ 
for the new components of vectors.

Trigger and associated particles can be chosen in various rapidity/pseudo-rapidity windows. Types
of the particles can or cannot coincide. It is useful to consider also the correlation functions
integrated on one or two variables.

Let us consider a connection of the functions with transverese momentum generation mechanism
(see Fig.~5).
Let us take a baryon ($\Lambda$) as a trigger particle. The transverse
momentum of the baryon ($\vec P^{\Lambda}$) is a sum of the transverese momentum of diquark 
($\vec  P_{qq}$) after previouse fragmentation steps and the transverse momentum of $s$-quark
($P_s$) produced from the vacuum: $\vec P^{\Lambda} =\vec  P_{qq}\ +\ \vec P_s$. The transverse momentum
of an associated hadron $\vec P^{as}=-\vec P_s\ + \vec P_q$. $\vec P_q$ is a transverse
momentum of a quark produced at the next fragmentation step from the vacuum.

\begin{minipage}{4cm} 5.5
%	\resizebox{2in}{2in}{\includegraphics{Fig1.png}}
	\resizebox{1.5in}{1in}{\includegraphics{Uzhinsk/GalUzhFig5.png}} % 2 1.75
	\centerline{Fig. 5} 
	\addtocounter{figure}{1}
	\label{Fig4}
	%	\addtocounter{figure}{1}
\end{minipage}
\begin{minipage}{8.5cm} % 7.4
According to the Schwinger's model \cite{Schwinger} implemented in the LUND fragmentation model \cite{LUND}
distributions of $\vec P_s$ and $\vec P_q$ are Gaussian ones. Assume for simplicity, that
distribution of $\vec  P_{qq}$ has also Gaussian shape. 

~~~~~~~~In the case, a probability density of the process is given by the expression:
\begin{equation}
W=
\left[\frac{1}{\pi\ \sigma_1}\ e^{-\vec P_{qq}^2/\sigma_1}\right] 
\left[\frac{1}{\pi\ \sigma_2}\ e^{-\vec P_{s}^2 /\sigma_2}\right] 
\left[\frac{1}{\pi\ \sigma_2}\ e^{-\vec P_{q}^2 /\sigma_2}\right]
\nonumber
\label{Eq11}
\end{equation} 
\end{minipage}

$$
\propto \exp(-\vec (P^{tr})^2/\sigma_1\ -\ \vec (P^{as})^2/\sigma_2\ +\ 
\frac{\sigma_1\ \sigma_2}{2 \sigma_1\ +\ \sigma_2}(\vec P^{tr}/\sigma_1 - \vec P^{as}/\sigma_2)^2).
$$

\noindent Choosing $x$-axis direction along the vector $\vec P^{tr}$, we have:  
\begin{equation}
W(\vec P^{tr},\vec P^{as})\ \propto\ \exp\left(-\frac{\sigma_1+\sigma_2}{\sigma_2 (2 \sigma_1+\sigma_2)}
\left[P^{as}_x+\frac{\sigma_2}{\sigma_1+\sigma_2} P^{tr}\right]^2 - 
\frac{\sigma_1+\sigma_2}{\sigma_2 (2 \sigma_1+\sigma_2)} (P^{as}_y)^2  \right)
\label{Eq13}
\end{equation}

Using Exp.~\ref{Eq13}, one can obtain for average values of projections of vector $\vec P^{as}$
on $x$ and $y$ axes the following expressions:  
\begin{equation}
<P^{as}_x>=-\frac{\sigma_2}{\sigma_1+\sigma_2} P^{tr},
\label{Eq14}
\end{equation}  
\begin{equation}
<(P^{as}_y)^2>=\frac{1}{2} \frac{2 \sigma_1+\sigma_2}{\sigma_1+\sigma_2}\cdot \sigma_2.
\label{Eq15}
\end{equation}

It is useful to consider the following cases:

$1)\ \ \sigma_1=0,\ \ \ <(P^{as}_y)^2>=\sigma_2/2,\ \ \ \ <P_{as,x}>=-P_{tr}$

$2)\ \ \sigma_1=\sigma_2,\  <(P^{as}_y)^2>=\frac{3}{4}\sigma_2,\ \ \ <P^{as}_x>=-\frac{1}{2}P^{tr}$

$3)\ \ \sigma_2\simeq 0,\ \ \ <(P^{as}_y)^2>\simeq 0,\ \ \ \ \ \ <P_{as,x}>\simeq 0$

In the first case, we assume that diquarks have no transverse momentum. The second case corresponds
to the assumptions that average momenta of quarks and diquarks are equal. The last one shows the
obvious results, when transverse momenta of sea quarks are equal zeros. 

%\subsection{Demonstration of the method}
Let us test the method on events generated by Pythia 6.4 and Geant4 FTF models 
at $\sqrt{s_{NN}}=$ 10 GeV. We chose for the testing $\Lambda$-hyperons as trigger particles, 
and considered anti-$\Lambda$ hyperons, $K$-mesons and $\pi$-mesons as associated particles.
We expected that there will be an essential difference between the model preductions due to the
difference in the baryon production mechanisms. As seen in Fig.~6, it is so. We present
in Fig.~6 $<P^{as}_x>$ as functions of triggered $\Lambda$ momentum for various associated
particles. 
\begin{figure}[bth]
\begin{center}
%% 22.12.2020
\resizebox{5in}{4.5in}{\includegraphics{Uzhinsk/GalUzhFig6.eps}} % 6 6.5
	\vspace{-3mm}
	\caption{$<P^{as}_x>$ as functions of triggered $\Lambda$ momentum for associated particles -- 
		$\bar \Lambda$, $K^0$, $K^+$, $K^-$, $\pi^+$ and $\pi^-$, figures {\it a, b, c, d, e} and {\it f},
		respectively, in $pp$ interactions at $\sqrt{s_{NN}}=$ 25 GeV. Open and filled symbols are Pythia 
		and FTF calculation results, respectively.}
\end{center}
\label{Fig6}
\vspace{-5mm}
\end{figure}

As seen, first of all, the correlations are approximately linear functions of  $P^{tr}$, as it was expected.  
A large deviation between the model results takes place for $\Lambda$ correlations with $\bar \Lambda$, 
$K^0$, $K^+$ and $\pi^-$ mesons. The models give close predictions for $\Lambda$ correlations with  
$K^-$ and $\pi^+$ mesons. In general, the FTF model predicts strongest correlations between
baryons and anti-baryons. Other strong correlations are between triggered $\pi$ mesons and baryons. The correlations
are weaker in the Pythia model. There is practically no correlations between $\Lambda$ and $\bar \Lambda$
hyperons in the Pythia model.  

According to the FTF model, there is an evolution of the correlations from strong to less strong ones
in the energy range $\sqrt{s_{NN}}=$ 3 -- 15 GeV. It is connected with dying out of the quark exchange 
processes in the FTF model. At higher energies the correlations become "frozen". A next step in 
the function's evolution can be at copious gluon production.

Correlations of $<(P^{as}_y)^2$ with $P^{tr}$ give a possibility of a direct check of the Schwinger's mechanism.
The correlations are presented in Fig.~7.

As seen, the correlations are practically constant. The model predictions are close to each other for $\pi^\pm$ and
$K^\pm$ mesons. There is an essential difference between the predictions for $\bar \Lambda$ hyperons and $K^0$ 
mesons. %According to the FTF model, there is a rising correlations between protons and $\pi$ mesons.

\begin{figure}[bth]
\begin{center}
%% 22.12.2020 
\resizebox{5in}{4.5in}{\includegraphics{Uzhinsk/GalUzhFig7.eps}}    % 6 6.5
	\vspace{-3mm}
	\caption{$<(P^{as}_y)^2>$ as functions of triggered $\Lambda$ momentum for associated particles -- 
		$\bar \Lambda$, $K^0$, $K^+$, $K^-$, $\pi^+$ and $\pi^-$, figures {\it a, b, c, d, e} and {\it f},
		respectively, in $pp$ interactions at $\sqrt{s_{NN}}=$ 25 GeV. Open and filled symbols are Pythia 
		and FTF calculation results, respectively.}
\end{center}
\label{Fig7}
%/\vspace{-5mm}
\end{figure}


The correlations evolve in the energy range $\sqrt{s_{NN}}=$ 3 -- 15 GeV in the FTF model. We believe all
of the considered correlations can be studied at the SPD experiment. 

%\newpage

%\nocite{*}
%\bibliographystyle{pepan}
%\bibliography{GalUzh}

%\end{document}

